Reinforcement Learning with Stepwise Fairness Constraints

AI methods are used in societally important settings, ranging from credit to employment to housing, and it is crucial to provide fairness in regard to algorithmic decision making. Moreover, many settings are dynamic, with populations responding to sequential decision policies. We introduce the study of reinforcement learning (RL) with stepwise fairness constraints, requiring group fairness at each time step. Our focus is on tabular episodic RL, and we provide learning algorithms with strong theoretical guarantees in regard to policy optimality and fairness violation. Our framework provides useful tools to study the impact of fairness constraints in sequential settings and brings up new challenges in RL.

==> RL with fairness constraint (Arxiv)/abs.tex <==
\begin{abstract}
AI methods are used in societally important settings, ranging from credit to employment to housing, and it is crucial to provide fairness in regard to algorithmic decision making. Moreover, many settings are dynamic, with populations responding to sequential decision policies.  We introduce the study of reinforcement learning (RL) with stepwise fairness constraints, requiring group fairness  at each time step. Our  focus is on tabular episodic RL, and we provide learning algorithms with strong theoretical guarantees in regard to policy optimality and fairness violation. Our framework provides useful tools to study the impact of fairness constraints in sequential settings and brings up new challenges in RL.
\end{abstract}

==> RL with fairness constraint (Arxiv)/conclusion.tex <==
\section{Conclusions}

==> RL with fairness constraint (Arxiv)/discussion.tex <==

\section{Discussion}
In this section, we discuss possible extensions of our framework and future directions.

%==============================
\subsection{Extension of stepwise fairness notions}\label{subsec:extfairnotion}
In our paper, we mainly consider two popular types of fairness criteria for stepwise fairness constraints, i.e. demographic parity and equalized opportunity. However, our techniques can also be extended in future work to additional types of fairness criteria. In particular, we can consider a family of fairness constraints, as formally introduced in \cite{agarwal2018reductions}. They consider constraints in the form 
$$M\mu(a)\le c$$ for matrix $M$ and vector $c$, where the $j$-th coordinate of $\mu$ is $\mu_j(a)=\bE[g(x,y,a,\vartheta)|E_j]$ for $j\in\mathcal{J}$, and $M\in\bR^{|\mathcal K|\times |\mathcal J|}$, $c\in\bR^{\mathcal K}$. Here, $\mathcal K=\cA\times\cY\times\{+,-\}$ ($+,-$ impose positive/negative sign so as to recover $|\cdot|$ in constraints), for $\cY=\{0,1\}$, and $\mathcal J=(\Lambda\cup \{*\})\times\{0,1\}$. $E_j$ is an event defined with respect to $(x,y,\vartheta)$ and $*$  denotes  the entire probability space. This formulation includes demographic parity and equalized opportunity as special cases. 


%==============================
\subsection{Aggregated fairness notions}\label{subsec:extfairnotion}
Despite the fact that we  consider stepwise fairness constraints, our techniques can also be extended in future work to aggregate fairness notions that consider the entire episodic process. Specifically, we could consider {\em aggregate equalized opportunity} (also called {\em aggregate true positive rate} in \cite{d2020fairness}):
$$\sum_{h=1}^H\bP(a_h=1|y_h=1,\vartheta)\frac{\bP(y_h=1|\vartheta)}{\sum_{h=1}^H\bP(y_h=1|\vartheta)},$$
which can be viewed as a weighted sum of equalized opportunity across steps. This should be relatively straightforward to handle through 
our techniques.

%==============================
\subsection{Non-episodic, infinite horizon Markov decision processes}
Another natural direction is to extend our framework to non-episodic infinite horizon. Taking DP as an example, we could consider
\begin{align*}
  &\qquad\quad\max_{\bpi\in\Pi_k}\sum_{h=1}^\infty \gamma^h\cR_{h} (\p,\bpi),\\
   &\qquad\qquad~~s.t.~~\forall h\in[H],\\
   &\gamma^h|\bP^{\pi^\alpha,p^{\alpha}}(a^\alpha_{h}=1)-\bP^{\pi^\beta,p^{\beta}}(a^\beta_{h}=1)|\le \hat c_{h}.
\end{align*}
This will involve using a more advanced version of concentration inequality for Markov chain, and we  leave this to future work.

==> RL with fairness constraint (Arxiv)/experiment.tex <==

\section{Experiments}
%\zhun{He, the notations are not consistent with previous sections.}
\paragraph{Settings.}
We take $H=8$ for each episode, and update our policy every 
$k=2^{l}$ episodes, where $l=3,4,\ldots, 18$. We update our policy in this non-linear way  for reasons of computational cost, i.e., to reduce the number of optimization problems we need to solve while still collecting a large quantity of data. 
%We use the exponential scale because we want to control the computational cost while collect as many data as possible (more data implies more accurate estimation by the counting method). 
We choose the relaxation parameters $\hat{c}_{k,h}$ and $\hat{d}_{k,h}$ as defined in the previous sections. %\dcp{add notation for relax param}. 
After each policy update, we use 8,000 episodes to evaluate the  new policy. We also produce confidence intervals by repeating each experiment five
times. 


%\dcp{how many episodes altogether?}
 %We run the training procedure with 10 updates of the policies. 
 %\dcp{so, 2560 episodes?}
%\dcp{episode seems very short given intepretation of one step per individual. will need some explanation/justification} 

\paragraph{Estimation and Optimization Process.}

%by point estimates and simple counting methods plus adding some bias-correcting terms in the very start. \dcp{can just say via standard MLE approach, and point to appendix?}
%\dcp{do you mean simulate or estimate? if estimate, I thought we were using the MLE/counting method?} 
%
%\paragraph{Optimization Procedure.}
%All the optimizations are composed of episodic return objective from two groups of people, fairness constraints from some fairness notions, conditional independence constraints, transition kernel constraints, probability box constraints, probability axiom constraint, and initial distribution constraints. 
\begin{figure*}[h!]
\centering

%\caption{Wasserstein Distances between non-synthetic and synthetic data for U.S. ETFs. \ref{fig_real_ret1} and \ref{fig_real_ret4} for asset returns; \ref{fig_real_invCov1} and \ref{fig_real_invCov3}  for estimated precision matrix; \ref{fig_real_portW1} and \ref{fig_real_portW3} for estimated portfolio weights. \label{fig2}}
\begin{subfigure}[b]{0.32\textwidth}
\centering
\includegraphics[width = \textwidth]{DpReal/DpRealGenerativeMix_linear_estConstr_policyUpdateAvgReward.png}
\caption{DP FICO Pareto ~~~~~~~~~ \label{DpRealGenerativeMix_linear_estConstr_policyUpdateAvgReward}}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
\centering
\includegraphics[width = 1\textwidth]{DpReal/DpRealGenerativeMix_linear_estConstr_trainEpisodeIndex.png}
\caption{DP FICO estConstr \label{DpRealGenerativeMix_linear_estConstr_trainEpisodeIndex}}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
\centering
\includegraphics[width = 1\textwidth]{DpReal/DpRealGenerativeMix_linear_policyUpdateAvgReward_trainEpisodeIndex.png}
\caption{DP FICO return \label{DpRealGenerativeMix_linear_policyUpdateAvgReward_trainEpisodeIndex}}
\end{subfigure}
\vskip\baselineskip
\begin{subfigure}[b]{0.32\textwidth}
\centering
\includegraphics[width = \textwidth]{EqOptReal/EqOptRealGenerativeMix_linear_estConstr_policyUpdateAvgReward.png}
\caption{EqOpt FICO Pareto ~~~~~~~~~ \label{EqOptRealGenerativeMix_linear_estConstr_policyUpdateAvgReward}}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
\centering
\includegraphics[width = 1\textwidth]{EqOptReal/EqOptRealGenerativeMix_linear_estConstr_trainEpisodeIndex.png}
\caption{EqOpt FICO estConstr ~~~\label{EqOptRealGenerativeMix_linear_estConstr_trainEpisodeIndex}}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
\centering
\includegraphics[width = 1\textwidth]{EqOptReal/EqOptRealGenerativeMix_linear_policyUpdateAvgReward_trainEpisodeIndex.png}
\caption{EqOpt FICO return \label{EqOptRealGenerativeMix_linear_policyUpdateAvgReward_trainEpisodeIndex}}
\end{subfigure}
$$\vspace{-0.5in}$$
\caption{FICO data result. \ref{DpRealGenerativeMix_linear_estConstr_policyUpdateAvgReward} and \ref{EqOptRealGenerativeMix_linear_estConstr_policyUpdateAvgReward} for Pareto frontier, \ref{DpRealGenerativeMix_linear_estConstr_trainEpisodeIndex}\ref{DpRealGenerativeMix_linear_policyUpdateAvgReward_trainEpisodeIndex} for the constraint violation level in the training dynamics  \ref{EqOptRealGenerativeMix_linear_estConstr_trainEpisodeIndex} \ref{EqOptRealGenerativeMix_linear_policyUpdateAvgReward_trainEpisodeIndex} for the avergage episodic return over the training dynamics. In Pareto plots, the point with cross marker is the result for the final episode. The text close to points stand for penalty parameters}
\end{figure*}

We estimate transition probabilities and rewards using the counting method outlined above. These estimates are used as the input for our algorithm.
The optimization problems are non-convex, and the detailed optimization formulations are included in Appendix~\ref{app:experiment}. We use Gurobi to solve, and set the optimality-value tolerance, feasibility tolerance, and solving time limit as 1e-3, 1e-6, and 300 seconds, respectively. We use the barrier algorithm for all problems. %\ref{Optimizations}. %\dcp{prob already have these earlier in paper? no need to repeat here}\\%For demographic parity, we have linear constraints with absolute value, and it can be converted to multiple linear constraints. For equal opportunity, we have fractional constraints with absolute value, which can be converted to multiple quadratic constraints. \dcp{if this is important, give more details here. if not, just defer entire paragraph to appendix}\\
%\dcp{maybe the occupancy measure approach will be introduced in this part of paper. if it is, then do it, and then explain this need for conditional independence of policy on $y$. else, just push all to appendix}
%We need to enforce conditional independence for $a$ and $y$ given $x$, i.e. $\bP(a_t = 1 | x_t=x,y_t=1, \vartheta_t=\vartheta) = \bP(a_t = 1 | x_t=x,y_t=0, \vartheta_t=\vartheta)$ to satisfy this POMDP setting. \\

%The initial distribution constraints are also enforced according to different initial empirical distribution from the data. \dcp{either formalize here, or just push all details to app}\\

%The original optimization problems for demographic parity with piecewise episodic return are nonconvex quadratic programming problems. The nonconvexity comes from the conditional independence constraints\\
%The surrogate optimization problems with demographic parity with piecewise episodic return and penalty terms are nonconvex quadratic programming problems. The nonconvexity comes from both the conditional independence constraints and penalty terms. \dcp{unless giving details here, can just push to app and say something like `The demo parity problem is a nonconvex quadratic program which we solve via xx , yy. }\\
%The original optimization problems for equal opportunity with piecewise episodic return are nonconvex quadratic programming problems. The nonconvexity comes from the conditional independence constraints and equal opportunity constraints.\\
%The surrogate optimization problems with equal opportunity with piecewise episodic return and penalty terms are nonconvex 4th order polynomial optimization problems. The nonconvexity comes from both the conditional independence constraints and penalty terms. We can convert it to quadratic optimization problem. \dcp{same comment}\\
%We also consider a risk sensitive setting, where the CARA utility serves as the episodic return, obtaining similar results as for the risk neutral setting (see Appendix \ref{Extended Experiment Results for concave risk sensitive episodic return}).
%For demographic parity, the conditional independence condition corresponds to a quadratic constraint. 

%, high numerical focus level, but do not use dual reduction 
 %\dcp{unclear... do not use, or use sometimes?}. 
%and translate the optimization problems into a bilinear form and use spatial branching. 

\paragraph{FICO Data.} We adapt FICO score data\footnote{\url{https://docs.responsibly.ai/notebooks/demo-fico-analysis.html}} to form
our data generating process. The FICO score dataset contains data from non-Hispanic White and Black cohorts consist of $j \in \cX=\{0, \ldots, 4\}$, which represent normalized score $\{0, 25, 50, 75, 100\}$ and can be viewed as the feature. In particular, the FICO data provides empirical  distributions for credit scores of different sensitive groups, i.e. $\hat{\bP}_{\text{FICO}}(x^\vartheta = j)$,  along with an empirical qualification distribution conditioned on each score level $\hat{\bP}_{\text{FICO}}(y^\vartheta = y|x^\vartheta = j)$, where $y\in\{0,1\}$. %%\dcp{give empirical details in Appendix?} %\dcp{explain $i$ for FICO data}
%\dcp{explain that we work with two groups, i.e., ... } 
%
We simulate the data generating process according to the empirical distributions stated above. For the population dynamics,  
we model the intial score distribution as
$\bP(x^\vartheta_0=j) = \hat{\bP}_{\text{FICO}}(x^\vartheta_0=j)$, according to
 the empirical  FICO distribution. %\dcp{how does this relate to FICO data?} 
For the initial qualification distribution conditioned on  score, 
$\bP(y^\vartheta_0=1|x_0=j)=\hat{\bP}_{\text{FICO}}(y^\vartheta = 1|x^\vartheta = j)$.
%again use the
%empirical FICO distribution.
 %\dcp{how does this relate to FICO data?} 
%
Then, we generate the underlying group-dependent and time invariant transition kernel $p^{*\vartheta}$ in the following way: we first set a distribution for $p^{*\vartheta}(x'=j'|x=j,y=w,a=v)$ for $j',j\in\cX$ and $w,v\in\{0,1\}$. Then, we set $p^{*\vartheta}(x',y'|x,y,a)$ as $p^{*\vartheta}(x'|x,y,a)\hat{\bP}_{\text{FICO}}(y^\vartheta = y'|x^\vartheta = x').$
%\begin{align*}
%p^{*\vartheta}(x_h=i|x_{h-1} \!=\! j, y_{h-1} \!=\! k, a_{h-1} \!=\! l)% \forall i,j,k,l%,\\
%p^\vartheta(x_h=i|x_{t-1} \!=\! j, y_{t-1} \!=\! 1, a_{t-1} \!=\! 0) &\!=\! g_{\vartheta,i,j, 1,0},\\
%p^\vartheta(x_h=i|x_{t-1} \!=\! j, y_{t-1} \!=\! 0, a_{t-1} \!=\! 1) &\!=\! g_{\vartheta,i,j, 0,1},\\
%p^\vartheta(x_h=i|x_{t-1} \!=\! j, y_{t-1} \!=\! 0, a_{t-1} \!=\! 0) &\!=\! g_{\vartheta,i,j, 0,0}.
%\end{align*}
%\dcp{as per earlier comment, could be written in concise form with index notation}
%Given the score sampled in the current step, 
%we have qualification status sampled from the distribution conditioning on the score of current step.
%$p^\vartheta(y_h=1|x_h=i) = f_{\vartheta,i}$, which also comes from empirical FICO distribution. %\dcp{why is this not the same as $f_{\vartheta,i}$?}
%\dcp{need to explain reward in FICO setting}
More details about the data generating process is specified in Appendix~\ref{app:experiment}.%~\ref{Semi-Realistic Data}. 

\paragraph{Reward function.} We choose a score-dependent reward, conditioned on the qualification level and decision as the following:
%We also assume the decision maker, for example a bank, receives more positive reward if they make a \dcpadd{positive decision} for a cohort with a higher score, e.g. making a good decision, but receive more negative reward if they make a \dcpadd{negative decision} for a cohort with a higher score. Moreover, The decision maker receives zero reward when they don't make a decision; i.e.,
%
\[
    r^\vartheta(x_h, y_h, a_h) =  
\begin{cases}
    \beta^\vartheta_1 x_h , & \text{if } y_h = 1, a_h = 1;\\
    -\beta^\vartheta_2 x_h , & \text{if } y_h = 0, a_h = 1;\\
    0,                    & \text{if } a_h = 0,
\end{cases}
\]
where $\beta^\vartheta_1, \beta^\vartheta_2 \in (0,1)$. Our reward function is chosen based on the following considerations: in real life, the decision maker may give a higher loan amount to a candidate with a higher credit score. As a result, the decision maker benefits more when a qualified candidate  has higher score, i.e. higher reward value (e.g. higher total repayment interests) gained from a qualified candidate with higher score because of higher loan amount; the decision maker also suffers more (more negative reward gained) if the candidate with higher score is not qualified, because a larger amount of loan is not repaid. In our experiment, we set $ \beta^\alpha_1=0.1, \beta^\beta_1=0.9, \beta^\alpha_2=0.9, \beta^\beta_2=0.1$. 
This difference in reward function per group further reflects a decision maker who may,  potentially irrationally and  unfairly, benefit or penalize through their reward function for different groups, even for two individuals who otherwise have the same score $x$ and qualification $y$ (perhaps the decision maker worries that the model is not equally accurate or calibrated per group).


%\dcp{as per above, notion of `cohort` and the way this specifies a `cohort score distribution` is unclear. even more so here, because you seem to be using FICO individual data yet talk about this modeling the adaptation of a cohort.}

%\dcp{need to also give specific parameter choices that you use in your experiments}


\paragraph{Baselines.}

We use the following policies as baselines:
%\begin{itemize}

1. Sequentially optimal policies without fairness constraints.
    %Policies based on an optimization without fair relaxation. In particular, in the optimization, the fairness notion related constraint is removed from the optimization formulation. 
    %

2. Sequentially optimal policies with an objective that includes a fairness penalty term, which serves as an alternative method for our proposed optimization problem. %(see the Appendix \ref{Optimizations}). 
   In this case, our optimization objective, for a particular kind of fairness constraint, is:
    %
    $$\max_{\bpi\in\Pi_k}\sum_{h=1}^H\left[ \cR_{k,h} (\p_k,\bpi)+\mathit{FP}(\{\pi^\vartheta,p^{\vartheta}_k,s^\vartheta_h,a^\vartheta_h\}_{\vartheta};\lambda)\right],$$
    where $\mathit{FP}(\{\pi^\vartheta,p^{\vartheta}_k,s^\vartheta_h,a^\vartheta_h\}_{\vartheta};\lambda)$ is the fairness penalty and $\lambda$ is the penalty parameter.
    \begin{itemize}
        \item[(a).] \textit{Demographic parity}. For this case, we choose $\mathit{FP}(\{\pi^\vartheta,p^{\vartheta}_k,s^\vartheta_h,a^\vartheta_h\}_{\vartheta};\lambda)$ as $$\lambda(\bP^{\pi^\alpha,p_k^{\alpha}}(a^\alpha_{k,h}=1)-\bP^{\pi^\beta,p_k^{\beta}}(a^\beta_{k,h}=1))^2.$$
        \item[(b).] \textit{Equalized opportunity.} For this case, we choose $\mathit{FP}(\{\pi^\vartheta,p^{\vartheta}_k,s^\vartheta_h,a^\vartheta_h\}_{\vartheta};\lambda)$ as
        \begin{align*}
\lambda\Big(&\bP^{\pi^\alpha,p_k^{\alpha}}(a^\alpha_{k,h}=1|y^\alpha_{k,h}=1)-\bP^{\pi^\beta,p_k^{\beta}}(a^\beta_{k,h}=1|y^\beta_{k,h}=1)\Big)^2
        \end{align*}
    \end{itemize}
   
 
 
    
%    \begin{align*}
%    \max_\rho\big [p_a\sum_{x,y,a,h}\rho^\alpha(x,y,a,h) \cR^{\alpha}_{(k)}(x,y,a) +\\ p_b\sum_{x,y,a,h}\rho^\beta(x,y,a,h) \cR^{\beta}_{(k)}(x,y,a)\big] \\
%    - \lambda \sum_{t,a}(\sum_{y,x} \rho^\alpha(x,y,a,h)-\sum_{y,x} \rho^\beta(x,y,a,h))^2
%    \end{align*}
    %\dcp{give math form of objective here} We use 0, 1, 10, 1000 as different penalty parameters. 
    %
%    \item A myopic policy, which uses a particular occupancy measure for each of the three cases (1) $y_h=1, a_h=1$, (2) $y_h=0, a_h=1$, and (3) $a_h=0$ (see the Appendix \ref{Myopic Policy baseline}). \dcp{need specifics here, and this is what we think is not implementable as an ``x, sens attribute only" policy. needs to be fixed.}


%\dcp{ideally we'd also have myopic + fairness}





\paragraph{Experimental results.}
Figure~\ref{DpRealGenerativeMix_linear_estConstr_policyUpdateAvgReward} shows the Pareto frontier in terms of episodic total return and episodic step-average fairness violation for demographic parity, and Figure \ref{EqOptRealGenerativeMix_linear_estConstr_policyUpdateAvgReward} shows the counterpart for equal opportunity.
%
Figure~\ref{DpRealGenerativeMix_linear_estConstr_trainEpisodeIndex} and~\ref{DpRealGenerativeMix_linear_policyUpdateAvgReward_trainEpisodeIndex} demonstrate the training dynamics of different algorithms
for demographic parity, and 
Figures~\ref{EqOptRealGenerativeMix_linear_estConstr_trainEpisodeIndex} and~\ref{EqOptRealGenerativeMix_linear_policyUpdateAvgReward_trainEpisodeIndex} demonstrate the counterpart
for equal opportunity.
%As with the synthetic data, 
Our proposed method outperforms the baselines in terms of Pareto frontiers, and converges to a stable level in terms of fairness violation over the training episodes. 
%\dcp{give a short summary.. it seems you're basically saying the same thing as above}
%
\if 0
We can our proposed method with snapshots from the training dynamics outperforms the surrogate penalty baseline with different penalty parameters and the myopic baselines with different parameters. \\over the episodes for demographic parity with respective to the episodic constraints and episodic return, respectively. We can see our algorithm converges after some episodes, and it achieves smaller episodic constraint and better episodic return than other methods. 
Figure \ref{EqOptRealGenerativeMix_linear_estConstr_policyUpdateAvgReward} shows the pareto frontier in terms of episodic return and episodic constraints for equal opportunity notion. We can our proposed method with snapshots from the training dynamics outperforms the surrogate penalty baseline with different penalty parameters and the myopic baselines with different parameters. \\
Figure \ref{EqOptRealGenerativeMix_linear_estConstr_trainEpisodeIndex} and Figure \ref{EqOptRealGenerativeMix_linear_policyUpdateAvgReward_trainEpisodeIndex} show the training dynamics over the episodes for equal opportunity with respective to the episodic constraints and episodic return, respectively. We can see our algorithm converges after some episodes, and it achieves smaller episodic constraint and better episodic return than other methods. \\
\fi
%
Overall, from the Pareto frontier, we can observe that our method reaches smaller fairness violation level for non-hispanic white and black individuals in both fairness notions, under a fixed reward level for the decision maker. In addition, from the confidence intervals, we can see that our algorithm has a much narrower confidence band than the other baseline.
%




==> RL with fairness constraint (Arxiv)/intro.tex <==
%=======================================================
\section{Introduction}
Decision making systems trained with real-world data are deployed ubiquitously in our daily life, for example, in regard to credit, education, and medical care. However, those decision systems may demonstrate discrimination against disadvantaged groups due to the biases in the data \cite{Dwork2012}. In order to mitigate this issue, many have proposed to impose fairness constraints \cite{hardt2016equality,Dwork2012} on the decision, such that certain statistical parity properties are achieved. Despite the fact that fair learning has been extensively studied, most of this work is in the static setting without considering the sequential feedback effects of decisions. At the same time, in many scenarios, algorithmic decisions may incur changes in the underlying features or qualification status of individuals, which further feeds back to the decision making process; for example, banks' decision may induce borrowers to react, for example changing their FICO score by closing  credit cards. 

When there exist sequential feedback effects, even ignoring one-step feedback effects can harm minority groups~\cite{liu2018delayed}. In response,~\cite{tu2020fair} advocates to study a discrete-time sequential decision process, where responses to the decisions made at each time step are accompanied by changes in the features and qualifications of the population in the next time step. In particular, they study and show the drawback of myopic optimization together with requiring fairness at each time step, which we  refer to as \textit{stepwise fairness constraints}. While imposing stepwise fairness constraints is a natural way to incorporate fairness into a Markov decision process (MDP), it makes more sense from the perspective of a decision maker to consider  the long-term reward. Thus, in this paper, we study stepwise fairness constraints together with optimal, sequential-decision making, taking the perspective of a forward-looking decision maker. On one hand, our work could be viewed as a {\em Fair Partially Observable Markov Decision Process} (F-POMDP) framework to promote fair sequential decision making \footnote{The problem of long-term well-being of groups brought up in \cite{liu2018delayed} is due to a misalignment of the institute's reward function and well-being measurements, and cannot be solved in any existing literature. It also doesn't prevent stepwise fairness constraints from being a way to build fair MDP.}. On the other hand, our work also provides a computational tool for studying the quantities of interests, such as well-being of groups, in a natural sequential decision making setting.
%dcp cut While imposing stepwise fairness constraints for a sequential decision making process may be one of the most straightforward ways to incorporate fairness into a dynamic decision making system, doing myopic optimization on rewards without considering long-term effect of decisions is not natural. It is more natural from the perspective of an institute to consider optimizing the long-term reward under stepwise fairness constraints. 
%

In particular, we initiate both the theoretical and experimental studies of reinforcement learning, i.e. optimizing long-term reward in a partially observable Markov decision process (POMDP), under stepwise fairness constraints. We consider an episodic setting, which models for example 
economic and societal activities that exhibit  seasonality; e.g., new mortgage applicants who 
apply for loans from banks more often in the spring and summer season every year, 
or  graduate school admission, which  usually starts in the
autumn and completes around December every year. 
%
%dcp cut Thus, decision receivers come to be served in a recurrent manner by decision makers, and it would be appropriate to model in an episodic manner. 
Similar to~\cite{liu2018delayed,tu2020fair}, we mainly consider two  types of fairness notions, \textit{demographic parity} and \textit{equalized opportunity}, and for a POMDP framework that has discrete actions and a discrete state space. These are illustrative of other stepwise fairness constraints that could be adopted. %Our framework is designed to maximize the utility of the decision maker while providing stepwise fairness. 
We take a model-based learning approach, and 
provide practical optimization algorithms that
enjoy strong theoretical guarantees  in regard to policy optimality and fairness violations
as the number of episodes increases. We summarize our contributions as below:

1. Theoretically, we demonstrate how to use sampled trajectories of individuals to solve RL with fairness constraints and provide theoretical guarantees to ensure vanishing regrets in reward and fairness violation as the number of episodes increases.

2. Experimentally, we implement the first algorithm for tabular episodic RL with stepwise fairness constraints.  



\subsection{Related work}
As the rapid development of machine learning \cite{he2016deep,he2017mask,goodfellow2020generative,deng2021adversarial,deng2021improving,deng2021toward,deng2020towards}, there is an increasing interest in the study of decision making problems in the context of people\cite{Hardt2015,Shavit2019,Ball2019,Chen2020,sun2020decision}. Hardt et al.~\cite{Hardt2015}
model a classification problem as a sequential game (Stackelberg competition) between two players, where the first player has the ability to commit to his strategy before the second player responds. They characterize the equilibruim and obtain near optimal computationally efficient learning algorithms.  Shavit and Moses~\cite{Shavit2019} study an algorithmic decision-maker who incentivizes
people to act in certain ways to receive a better decision.
%\dcp{and show ...}. 
Ball et al.~\cite{Ball2019} study a model of predictive scoring, 
%which composed of three players: sender, intermediary, and receiver. The 
where there is a sender agent being scored, a receiver agent who 
wants to predict the quality of the sender, and an
intermediary who observes multiple, potentially mutable features of the sender.
%\dcp{maybe go with hardt et al first, since they introduced this, and say more about their model. also, chara podimata has worked on this, I think} 
%\dcp{ for hardt et al, prob should try to say what is similar/different from our setting}

There is also a growing literature on algorithmic fairness~\cite{liu2018delayed,Calders2009,Kusner2017,Dwork2012,deng2022fifa,deng2020representation,burhanpurkar2021scaffolding,zhang2022and,deng2020interpreting}.
%
%\dcp{add a bunch of cites, prob grouping into group-based as in the present paper, and individual}. 
Liu et al.~\cite{liu2018delayed}, for example, characterize the delayed impact of standard fairness criteria
under a feedback model with a single period of adaptation. They use a one step feedback model to capture the sequential dynamics of the environment. 
%\dcp{unclear, say more about how same/different from this paper}. 
However, these papers do not consider the fairness in a more general sequential decision process. %\dcp{say more to explain why liu et al don't}
There is also  a line of literature regarding fair bandits, but not more general (PO)MDP problems~\cite{Joseph2016,Hashimoto2018}.
%However, their optimal policy is always fair, thus solving the optimal fair policy is trivial. 
%
%\dcp{this is where we'll want to cite the fair bandits work, e.g., aron roth, yang liu, etc and the fair RL paper I shared, and anything else relevant. cite and contrast.} 
In regard to fairness considerations in reinforcement learning, it has also gained great attention~\cite{DAmour2020,Creager2019,Wen2021,Jabbari2017,Mandal2022,deng2021improving,kawaguchi2022understanding,deng2021toward}. In particular, Creager et al.~\cite{Creager2019} use  causal directed acyclic graphs as a unifying framework for fairness. D'Amour et al.~\cite{DAmour2020} use simulation to study the fairness of algorithms and  show that neither static nor single-step analyses is  enough to
 understand the long-term consequences of a decision system.
Jabbari et al.~\cite{Jabbari2017} 
define fairness constraints to require that an algorithm never prefers one action over another if the long-term reward of choosing the latter action is higher, whereas we consider groupwise notions of fairness. 
%\dcp{explain how this is similar/different to what you do}
Mandal et al.~\cite{Mandal2022} adopt a welfare-based, axiomatic approach, and give a regret bound for the Nash Social, Minimum and generalized Gini Welfare. 
%They have fairness notion in terms of different type of welfares. 
In contrast with our work, the fairness concepts are not group-based but rather based on the value contributed from different agents in the system. % \dcp{what?}.
%
Similar to this paper, Zhang et al.~\cite{Zhang2020}
study the dynamics of population qualification and algorithmic decisions under
a partially observed Markov decision problem setting, but whereas they 
only consider myopic policies, we frame this as a
general reinforcement learning policies. 
%
%In this paper, we model group-wise fairness notions in a POMDP framework and propose optimization based policies with theoretical guarantees. 




==> RL with fairness constraint (Arxiv)/preliminary.tex <==
%=======================================================

\section{Preliminaries}

%In this section, we  introduce the notations, fairness notions, and expected reward we consider in this paper. Our notations and terminologies will mostly be adopted from reinforcement learning for consistency.

%=============
We consider a binary decision setting, with training examples that consist of triplets $(x, y, \vartheta)$, where $x\in\cX$ is a feature vector, $\vartheta\in \Lambda$ is a protected group attribute such as race or gender, and the label $y\in\{0,1\}$.% is an individual's qualification status. 
For simplicity, we only consider binary sensitive attributes $\Lambda=\{\alpha,\beta\}$, but our method can also be generalized to deal with multiple sensitive attributes (see Appendix~\ref{app:multipleatt}).
For $k\in \bN^+$, we use $[k]$ to denote the set $\{1,2,\cdots,k\}$. 

Based on feature $x$, a decision maker makes a decision $a\in\cA=\{0,1\}$ (e.g., make a loan or not). We will also denote an individual's state as $s=(x,y)$, and let $\cS=\cX\times\cY$.  After a decision is made, a possibly group-dependent reward, which may be stochastic, $r^\vartheta: (s,a)\mapsto \bR$ is obtained by the decision maker. %\dcp{no need to say `unknown`}
%
A concrete  example of a reward function, with  $r_+,r_->0$,  is 
%
$$
r^\vartheta(s,a)=\left\{\begin{matrix}
r_+, &\mbox{if $y=1,a=1$;}\\ 
	-r_-,&\mbox{if $y=0,a=1$;}  \\
	0, &\mbox{if $a=0$.}
\end{matrix}\right.$$

Here, the decision maker gains $r_+$ by accepting a qualified individual and incurs a cost $r_-$ by accepting an unqualified individual. 

%For two positive sequences $\{\xi_k\}$ and $\{\eta_k\}$, we write $\xi_k =O(\eta_k)$ (or $\xi_k\lesssim \eta_k$), and $\xi_k = o(\eta_k)$, if $\lim_{k\rightarrow\infty}(\xi_k/\eta_k) < \infty$ and $\lim_{k\rightarrow\infty}(\xi_k/\eta_k) =0$ respectively. $\tilde O(\cdot)$ denotes the term, neglecting the logarithmic factors. We also write $\xi_k=\Theta(\eta_k)$ (or $\xi_k\asymp \eta_k$) if $\xi_k\lesssim \eta_k$ and $\eta_k\lesssim \xi_k$. We use $O_p(\cdot)$ to denote stochastic boundedness: a random variable $z_k=O_p(\xi_k)$ for some real sequence $\xi_k$ if $\forall \epsilon>0$, there exists $M,N>0$ such that if $k>N$, $\bP(|z_k/\xi_k|>M)\le \epsilon$.
\iffalse
%=============
\textbf{Basic fairness notions.} We mainly work with two widely used group fairness definitions; however, our approach can also be extended to additional fairness notions (see Section \ref{subsec:extfairnotion}). Specifically, we consider the following two kinds of  fairness. 

(i). \textit{Demographic Parity (DP)}. The action $a$ satisfies demographic parity if $a$ is statistically independent of the sensitive attribute $\vartheta$: $$\bP(a=1|\vartheta=\alpha)=\bP(a=1|\vartheta=\beta).$$
(ii). \textit{Equality of Opportunity (EqOpt)}.  The action $a$ satisfies equality of opportunity if $a$ is conditionally independent of the sensitive attribute $\vartheta$ given $y=1$:
	$$\bP(a=1|y=1,\vartheta=\alpha)=\bP(a=1|y=1,\vartheta=\beta).$$
	\fi
%=============

\subsection{Sequential setting}

%\textbf{Expected reward of a random individual.} In this paper, our aim is to 

%We propose reinforcement learning methods for general reward functions and along with
%different kinds of fairness constraints. %In this paper, each group $\vartheta$ has its own (possibly unknown and stochastic) reward function $r^\vartheta: (x,y,a)\mapsto \bR$, 
%


Our model as a partially observable Markov decision process (POMDP) mainly follows~\cite{tu2020fair}, but they consider a fair, myopically-optimizing policy while we consider long-term rewards as in typical RL settings. 
Following~\cite{liu2018delayed,tu2020fair}, the decision maker is
interested in the expected reward 
achieved across time for a \textit{\textbf{random individual}} drawn from the population.
%
Each random individual has their group membership sampled according to 
$p_\alpha=\bP(\vartheta=\alpha)$ and $p_\beta=\bP(\vartheta=\beta)$, and interacts with the decision maker over multiple time steps.
% Specifically, we assume that at time $h=1$
%
%
At each time step $h$, the sampled individual with attribute $\vartheta$ has feature $x^\vartheta_h=x^\vartheta \in\cX$ along with a hidden qualification status $y^\vartheta_h=y^\vartheta \in\{0,1\}$. One example is that the feature $x^\vartheta_h$ is determined by the hidden qualification status with $x^\vartheta_h\sim p(\cdot|y^\vartheta)$. 
%
We call $s^\vartheta_h=(x^\vartheta_h,y^\vartheta_h)$ the 
{\em state } 
of the individual at time $h$. 
The initial state $s^\vartheta_1$ is sampled from $p^\vartheta$.

At each time step $h$, the 
decision maker adopts a decision $a^\vartheta_h$  based on the observed feature $x^\vartheta$ by following a {\em group-dependent policy} $\pi^\vartheta_h(x^\vartheta)$, i.e. $a^\vartheta_h\sim \pi^\vartheta_h(x^\vartheta_h)$, where $\pi^\vartheta_h:\cX\rightarrow\Delta(\cA)$, and $\Delta(\cA)$ is the set of distributions on $\cA$.\footnote{Following~\cite{tu2020fair}, 
we use group-dependent policies so that the formulation can be more generalized. Our technique can also be used for group-independent policies if this is required.}
%
%the ideal optimization problem is using  approximate fairness with suitable relaxations.  \zhun{I am skeptical of this motivation in \cite{tu2020fair}}}. 
%
The decision maker receives 
{\em reward} $r^\vartheta(s^\vartheta_h,a^\vartheta_h)$, and $r^\vartheta\in[l,u]$, where $-\infty<l-u< \infty$. Without loss of generality, let us assume $r^{\vartheta}\in[0,1]$. The mean of stochastic reward function is denoted by $r^{*\vartheta}$.

After the decision is made, the individual is informed of the decision and their qualification status,  and  their qualification status, $y^\vartheta_{h+1}$, and features $x^\vartheta_{h+1}$, may
then undergo a stochastic transition.
 %
 We assume that this transition follows
 a {\em time-invariant} but {\em group-dependent transition kernel},
which we denote as 
$p^{*\vartheta}(s^\vartheta_{h+1}|s^\vartheta_h,a^\vartheta_h)$, where $p^{*\vartheta}:\cS\times \cA\mapsto \Delta(\cS)$, and $\Delta(\cS)$ is the set of distributions on $\cS$. 
 %
 As explained in~\cite{tu2020fair}, in addition to thinking about a single, randomly chosen individual 
 repeatedly interacting with the decision maker, this also immediately models a finite population of randomly chosen individuals, some from each group, and with all individuals in a group
 subject to the same, group-contingent decision policies. In addition, we have a reward function pair, $(r^{\alpha},r^{\beta})$, 
 which may be stochastic. 

%\dcp{don't think we need this, and it's also confusing, because it fixes the state before sampling the individual, which seems backwards}

%the expected reward of a random individual is defined as:
%\begin{align*}
%	\cR(s,a)=\sum_{\vartheta\in\{\alpha,\beta\}}p_\vartheta\cdot  \bE[r^\vartheta(s,a)|\vartheta].
%\end{align*}



%=======================================================
%\subsection{Sequential setting}\label{subsec:sequential}

%\textbf{Partially Observed Markov Decision Process.}
%\zhun{To do: $
%\bE^{\pi,p}$ needs more refined definition.} \zhun{I incorporate David's opinions about multiple individuals in the data gathering part, because section 2 is just about a single randomly drawn individual} 



%
%We have two groups, $\cG_\alpha$ and $\cG_\beta$, each with fraction %$\{p_\vartheta\}_{\vartheta\in\{\alpha,\beta\}}$. 
%

 
 \subsection{Fair policies}
 
 The goal of the decision maker is to   find a {\em policy}, $\bpi=(\pi^\alpha,\pi^\beta)$, to
 maximize the total, expected reward over an episode   for a random individual, while satisfying stepwise fairness constraints, i.e. imposing a certain type of fairness constraint on states and actions for each time step.
 %, so as to ensure fairness for decisions
 % for a randomly drawn individual in
 % each step, according to different fairness concepts.
  
  %Specifically, let $\bE^{\pi,p},\bP^{\pi,p}$ be the expectation and probability over the run of any policy pair $\bpi=(\pi^\alpha,\pi^\beta)$ and transition probability pair $\p^{*}=(p^{*\alpha},p^{*\beta})$. 
  
A random individual   in group $\vartheta$, and with decision policy $\pi^\vartheta$,  follows
stochastic state, action, reward sequence $s^\vartheta_1,a^\vartheta_1,r^\vartheta(s^\vartheta_1,a^\vartheta_1),s^\vartheta_2,a^\vartheta_2,r^\vartheta(s^\vartheta_2,a^\vartheta_2),s^\vartheta_3,\cdots$.
%
%
%following $\pi^\alpha$ and $p^{*\alpha}$, this individual produces a stochastic trajectory on states and actions, i.e. $\{s^\alpha_h,a^\alpha_h,r^\alpha(s^\alpha_h,a^\alpha_h)\}_{h}$. Similar for the case that the individual belongs to $\cG_b$, the individual can produce a stochastic trajectory following $\pi^\beta$ and $p^{*\beta}$, i.e. $\{s^\beta_h,a^\beta_h, r^\beta(s^\beta_h,a^\beta_h)\}_{h}$. 
%\fi
%
%The decision maker wants to 
%to optimize the long-term reward while ensuring a certain type of fairness constraint on $(s^\alpha_h,a^\alpha_h)$ %and $(s^\beta_h,a^\beta_h)$ is satisfied for all $h$ over a period with total $H$ time steps. 
%
%
Let $\bE^{\pi,p}[\cdot],\bP^{\pi,p}[\cdot]$ be the expectation and probability of a random variable defined with respect to this stochastic process.
%
%over the run of any policy $\pi$ and transition kernel $p$. 
%
We denote the expected reward for a random individual at time step $h$  as,
%
$$\cR^*_h(\p^*,\bpi)=\sum_{\vartheta\in\{\alpha,\beta\}}p_\vartheta\cdot  \bE^{\pi^\vartheta,p^{*\vartheta}}[r^{*\vartheta}(s^\vartheta_h,a^\vartheta_h)].$$
%\begin{align*}
%	\cR^*_h(\p^*,\bpi)=\sum_{\vartheta\in\{\alpha,\beta\}}p_\vartheta \bE^{\pi^\vartheta,p^{*\vartheta}}[r^{*\vartheta}(s^\vartheta_h,a^\vartheta_h)].
%\end{align*}

%\dcp{I think the above needs the expectation to be conditioned on the sensitive attribute of the individual in period 1 being $\vartheta$.}
Note here that $\bE^{\pi^\vartheta,p^{*\vartheta}}[\cdot]$ refers to the expected value for an individual in group $\vartheta$, i.e.,
conditioned on the individual being sampled in this group.
Our ideal goal is to obtain the  policy  $\bpi^*$ that solves the following optimization problem:
%
\begin{align*}
&\qquad\quad\max_{\bpi}\sum_{h=1}^H \cR^*_h (\p^*,\bpi)\\
  &\qquad\qquad \mbox{s.t.}~~\forall h\in[H],  \\
  &\mathit{faircon}(\{\pi^\vartheta,p^{*\vartheta},s^\vartheta_h,a^\vartheta_h\}_{\vartheta=\{\alpha,\beta\}}),
\end{align*}
%
%$$\max_{\bpi}\sum_{h=1}^H \cR^*_h (\p^*,\bpi),$$
 %  $$ s.t.~~\forall h\in[H],$$
  % $$faircon(\{\pi^\vartheta,p^{*\vartheta},s^\vartheta_h,a^\vartheta_h\}_{\vartheta=\{\alpha,\beta\}})$$
where $\mathit{faircon}$ corresponds to a particular fairness concept.
%
We consider two group fairness definitions, and also discuss how the approach can be  extended to additional fairness concepts (see Section~\ref{subsec:extfairnotion}).
%
Specifically, we consider the following two   fairness concepts: 

(i) \textit{RL with demographic parity (DP)}. For this case,  $\mathit{faircon}$ is%$$\max_{\bpi}\sum_{h=1}^H \cR^*_h (\p^*,\bpi),$$
   %$$ s.t.~~\forall h\in[H],$$
   $$\quad\bP^{\pi^\alpha,p^{*\alpha}}[a^\alpha_h=1]=\bP^{\pi^\beta,p^{*\beta}}[a^\beta_h=1],$$
   %
   which means at each time step $h$, the decision for individuals from different groups is  statistically independent of the sensitive attribute.
   %\dcp{I think the above needs the prob to be conditioned on the sensitive attribute of the individual in period 1 being $\alpha$ and $\beta$, respectively.}
   
(ii) \textit{RL with equalized opportunity (EqOpt)}. For this case, $\mathit{faircon}$ is%$$\max_{\bpi}\sum_{h=1}^H \cR^*_h (\p^*,\bpi),$$ $$s.t.~~\forall h\in[H],$$
    $$\bP^{\pi^\alpha,p^{*\alpha}}[a^\alpha_h=1|y^\alpha_h=1]=\bP^{\pi^\beta,p^{*\beta}}[a^\beta_h=1|y^\beta_h=1],$$
%\end{itemize}
which means at each time step $h$, the decision for a random individual from
each of the two different groups is  statistically independent of the sensitive attribute conditioned 
on the individual being qualified.
 %\dcp{I think the above needs the prob to be conditioned on the sensitive attribute of the individual in period 1 being $\alpha$ and $\beta$, respectively.}
In each case, $\bP^{\pi^\alpha,p^{*\alpha}}[\cdot]$ refers to the probability for an individual in group $\vartheta$, i.e.,
conditioned on the individual being sampled in this group.

The above optimization problems are feasible under technical Assumption~\ref{ass:kernel}, presented later, and we assume feasibility throughout the paper (see also Appendix~\ref{app:feasibility}). %The above problems are always feasible under some conditions such as $p^{*\vartheta}(s'|s,a)\neq 0$ for all $s,a,s'$. In this paper, all the discussions are only for feasible cases.

\begin{remark}
Since we are modelling the behavior of a randomly drawn individual from the population, the objective  should be viewed as to find a policy pair $\bpi=(\pi^\alpha,\pi^\beta)$ to optimize the long-term reward of 
of the decision maker while ensuring fairness over the population. %we learn different policies for individuals from different demographic groups respectively. For each demographic group, the aim is to learn a single policy for all individuals from the group, so that the learned policy pair for the two groups can maximize the expected reward for a random individual drawn from the population. However, the data is gathered from multiple individuals from each demographic group, as we will show in Section \ref{sec:EFH algo}.
\end{remark}

\subsection{Episodic RL protocol} 
This is a learning setting, and we study an
episodic sequential decision setting where
a learner  repeatedly   interacts with an environment
across $K>0$  independent episodes.
%
%
Such a scenario is natural in a number of practical settings, as we discussed in the introduction.
%
%Similar to~\cite{brantley2020constrained}, the environment includes the state space $\cS$, the action space $\cA$, and the episode horizon $H$. 
%
Throughout the paper, we consider the tabular case, i.e., we assume finite cardinality for $\cS$ and $\cA$.\footnote{In the example of credit score and loan payment in \cite{liu2018delayed}, the credit score is discretized and served as $\cX$ here and the action space $\cA$ and qualification status space $\cY$ are both $\{0,1\}$.}
%which perfectly satisfy the tabular setting.
%
Without loss of generality, we can assume 
that the initial state of an episode is a fixed state $s_0$ (the next state can be sampled randomly, and  state $s_0$ does not contribute to any reward or fairness considerations, see \cite{brantley2020constrained} for further detailed explanation).
%
%
%Recall in our setting we have an unknown underlying transition probability pair $\p^*=(p^{*\alpha},p^{*\beta})$, each for a different demographic group. The institute is tracking the feedback and the expected reward for a random individual drawn from the population. %One concrete example of the learner is a bank, and the bank is tracking the loan pay-off of the population. When an individual pay-off his/her loan, there is a positive reward. The bank is tracking the average reward of the population, which is equivalent to tracking the expected reward for a random individual drawn from the population. 
%
%Since the drawn individual can either be from $\cG_\alpha$ or $\cG_\beta$, we can consider 
%
At episode $k\in[K]$, denote policy pair $\bpi_k=(\pi^\alpha_k,\pi^\beta_k)=\{(\pi^\alpha_{k,h},\pi^\beta_{k,h})\}_{h=1}^H$, where $H$ is the horizon.
%and $\pi^\vartheta_{k,h}:\cX\mapsto \Delta(\cA)$ corresponds to the policy of demographic group $\vartheta$ and specifies how to choose actions at step $h$ of for every feature vector $x$. 
%
An individual sampled from group $G_\vartheta$ starts from state $s^\vartheta_{k,1}$, thus, we can consider starting state pair $(s^\alpha_{k,1}, s^\beta_{k,1})=(s^\alpha_0,s^\beta_0)$ for the trajectory of different groups (the initial state depends on the group from which the individual is drawn). At each time step $h\in [H]$,
%for $s^\vartheta_{k,h}$, 
the decision maker selects an action $a^\vartheta_{k,h}\sim \pi^\vartheta_{k,h}(x^\vartheta_{k,h})$.
Here, although the policy only uses the $x$ component, it is convenient to write it as a function of $s$.
The decision maker gets  reward $r^\vartheta(s^\vartheta_{k,h},a^\vartheta_{k,h})$, and the state of the individual for next time step is drawn according to $s^\vartheta_{k,h+1}\sim p^{*\vartheta}(\cdot|s^\vartheta_{k,h},a^\vartheta_{k,h})$.

\begin{remark}
The policy is only based on the  \textit{\textbf{feature vector}} $x$. However, we are able to access $y$ in the training data.
\end{remark}











==> RL with fairness constraint (Arxiv)/theory.tex <==
%==========================================
\section{Learning Algorithms}\label{sec:EFH algo}

Before we formally state our algorithms, we need to gather data to estimate the unknown quantities such as reward function mean pair $\br^*=(r^{*\alpha},r^{*\beta})$ and transition probability pair $\p^*$. In addition, we will incorporate an {\em exploration bonus} to further modify the estimation.

%=============
\paragraph{Data gathering and estimation.} 
In order to analyze the policy effect on the population, we model the behavior of a randomly drawn individual who interacts with the environment across $H$ steps. Here, we demonstrate how to aggregate individuals' data   for each episode and estimate quantities of interest. Specifically, at episode $k\in[K]$, for each group $\vartheta$, we assume  $n^\vartheta_{k}$  individuals are drawn, according to $p_\alpha$ and $p_\beta$. Throughout the paper, we assume $n^\vartheta_k\ge 1$, for each $\vartheta$ and $k$. 
%For simplicity, we assume those individuals interact with the environment repeatedly during this episode. 
A decision is made independently for each individual at each step, using a group-specific policy, leading to a stochastic transition in the state of the individual. In Appendix~\ref{app:optin}, we will further discuss how to gather data when allowing individuals who opt in or out 
during an episode. We use the counting method to obtain estimates of the statistics of interest.  For the $i$-th individual in episode $k$, their status and action at time step $h$ is denoted as $s^{\vartheta,(i)}_{k,h}$ and $a^{\vartheta,(i)}_{k,h}$. 

For $\vartheta\in\{\alpha,\beta\}$, let $\p_k=(p^\alpha_k,p^\beta_k)$ and $\br_k=(r^\alpha_k,r^\beta_k)$, 
\begin{align*}
N^\vartheta_{k}(s,a)&=\max\big\{1, \sum_{t\in [k-1],h\in[H],i\in[n^\vartheta_k]} \mathbbm{1}\{s^{\vartheta,(i)}_{k,h}=s,a^{\vartheta,(i)}_{k,h}=a\}\big\},\\
p^\vartheta_{k} (s'|s,a)&=\frac{1}{N^\vartheta_{k}(s,a)}\sum_{t\in [k-1],h\in[H],i\in[n^\vartheta_k]} \mathbbm{1}\{s^{\vartheta,(i)}_{k,h}=s,a^{\vartheta,(i)}_{k,h}=a, s^{\vartheta,(i)}_{k,h+1}=s'\},\\
%$$p^s_{(k)} (y|x)=\frac{1}{N^s_{k}(x)}\sum_{j\in [k-1],t\in[T]} \mathbf{1}\{x^s_{j,t}=x, y^s_{k,t}=y\},$$
\hat{r}^\vartheta_{k} (s,a)&=\frac{1}{N^\vartheta_{k}(s,a)}\sum_{t\in [k-1],h\in[H],i\in[n^\vartheta_k]}r^\vartheta(s,a)\mathbbm{1}\{s^{\vartheta,(i)}_{k,h}=s,a^{\vartheta,(i)}_{k,h}=a\}.
\end{align*}






%=============
\paragraph{Exploration bonus method.} In RL, it is standard to introduce optimism in order to encourage exploring under-explored states. Specifically, for $\vartheta\in\{\alpha,\beta\}$, we adopt a {\em bonus term}, $\hat{b}^\vartheta_k$, to add to the estimated reward function $\hat{r}^\vartheta_{k}$, such that we obtain $r^\vartheta_{k}(s,a)=\hat{r}^\vartheta_{k}(s,a)+\hat{b}^\vartheta_{k}(s,a)$, where the $\hat{b}^\vartheta_{k}(s,a)$ values assign larger values for under-explored $(s,a)$'s. We  specify how to choose $\hat b^\vartheta_k$ in Section \ref{subsec:theory}, and  denote
%
\begin{equation*}
	\cR_{k,h}(\p,\bpi)= \sum_{\vartheta\in\{\alpha,\beta\}} p_\vartheta\cdot \bE^{\pi^\vartheta,p^{\vartheta}}[r_k^{\vartheta}(s^\vartheta_{k,h},a^\vartheta_{k,h})].
\end{equation*}

%
For the purpose of analysis, we  treat $p_\vartheta$'s  as known constants for simplicity; for example, perhaps these proportions  are provided by census.

%=============
\textbf{Practical optimization for DP.} In reality, given we don't have access to $\p^*$ and $r^{*\vartheta}$, we need to solving a surrogate optimization problem and hope the optimal policy can have similar performance as the ideal optimal policy under certain performance criteria. In the following, we provide a simple algorithm for RL with demographic parity. It is based on optimization under $p^{\vartheta}_k$ and $r^{\vartheta}_k$:
\begin{align*}
  &\qquad\quad\max_{\bpi\in\Pi_k}\sum_{h=1}^H \cR_{k,h} (\p_k,\bpi),\\
   &\qquad\qquad~~s.t.~~\forall h\in[H],\\
   &|\bP^{\pi^\alpha,p_k^{\alpha}}(a^\alpha_{k,h}=1)-\bP^{\pi^\beta,p_k^{\beta}}(a^\beta_{k,h}=1)|\le \hat c_{k,h},
\end{align*}
 %$$\max_{\pi\in\Pi_k}\sum_{h=1}^H \cR_{k,h} (\p_k,\bpi),$$
   %$$ s.t.~~\forall h\in[H],$$
  % $$|\bP^{\pi^\alpha,p_k^{\alpha}}(a^\alpha_{k,h}=1)-\bP^{\pi^\beta,p_k^{\beta}}(a^\beta_{k,h}=1)|\le \hat c_{k,h},$$
where we have $\Pi_k=\{(\pi^\alpha,\pi^\beta): \pi^\vartheta(a=1|x)\ge \eta^{\mathit{DP}}_k,\forall x,a,h,\vartheta\}.$ $\Pi_k$ can ensure the reachability from any $x$ to the decision $a=1$. Here $\{\eta^{\mathit{DP}}_k\}_k$ is a sequence of real numbers and $\{\hat c_{k,h}\}_{k,h}$ are relaxations.
Intuitively, if we set $\eta^{\mathit{DP}}_k$ and $\hat c_{k,h}$ to be decreasing and vanishing as $k$ increases, we would expect the above optimization  to approach the ideal optimization problem as $k$ increases. We formalize this in Section \ref{subsec:theory}. 

%\begin{remark}
%About the constraint over $\pi\in\Pi_k$, for simplicity, we assume it is feasible throughout our paper. Notice this assumption can be satisfied when, but much weaker than, requiring $p^\vartheta_k(s'|s,a)\neq 0$ for all $s',s,a$.
%\end{remark}







%=============
\paragraph{Practical optimization for EqOpt.} For equalized opportunity, and similar to the case of DP, we have
 \begin{align*}
  &\qquad\qquad\max_{\pi\in\Pi_k}\sum_{h=1}^H \cR_{k,h} (\p_k,\bpi),\\
  &s.t.~~\forall h\in[H],~~|\bP^{\pi^\alpha,p_k^{\alpha}}(a^\alpha_{k,h}=1|y^\alpha_{k,h}=1)-\bP^{\pi^\beta,p_k^{\beta}}(a^\beta_{k,h}=1|y^\beta_{k,h}=1)|\le \hat d_{k,h},
 \end{align*}
   %\begin{align*}
%s.t.~~\forall h\in[H],~~&|\bP^{\pi^\alpha,p_k^{\alpha}}(a^\alpha_{k,h}=1|y^\alpha_{k,h}=1)\\
%&-\bP^{\pi^\beta,p_k^{\beta}}(a^\beta_{k,h}=1|y^\beta_{k,h}=1)|\le \hat d_{k,h}
 %  \end{align*}
%   $$|\bP^{\pi^\alpha,p_k^{\alpha}}(a^\alpha_{k,h}=1|y^\alpha_{k,h}=1)-\bP^{\pi^\beta,p_k^{\beta}}(a^\beta_{k,h}=1|y^\beta_{k,h}=1)|\le \hat d_{k,h},$$
where  we have $\Pi_k=\{(\pi^\alpha,\pi^\beta): \pi^\vartheta(a=1|x)\ge \eta^{\mathit{EqOpt}}_k,\forall x,a,h,\vartheta\}.$
Here $\{\eta^{\mathit{EqOpt}}_k\}_k$ is a sequence of real numbers and $\{\hat d_{k,h}\}_{k,h}$ are relaxations. We formalize this in Section \ref{subsec:theory}.   

\paragraph{Algorithm.} We can solve these optimization problems through  occupancy measures, and they each become different kinds of quadratically constrained linear programs (QCLP) (see Appendix~\ref{app:occupancy}). 
%
Although QCLP is generally NP-hard, many methods based on relaxations and approximations such as semi-definite program (SDP) have been extensively discussed. We use Gurobi to solve these relaxed optimization problems.
%dcp cut , redundant given above The above optimization problems are feasible under Assumption~\ref{ass:kernel} and we assume feasibility throughout the paper. We defer the detailed discussion of feasibility in Appendix~\ref{app:feasibility}.

%==========================================
\section{Theoretical Analysis}

%\textbf{Criteria to measure performance.} 

In order to track the performance, we consider the following regrets. For policy pairs $\{\bpi_k\}_{k=1}^K$, for {\em reward regret} in episode $k$, we  track:
$$\cR^{\text{type}}_{\mathrm{reg}}(k)= \frac{1}{H}\sum_{h=1}^H\Big(\cR^*_h (\p^*,\bpi^{*\text{type}})-\sum_{t=1}^k\cR^*_h (\p^*,\bpi_k)\Big),$$
where $\bpi^{*\text{type}}$ is the optimal policy pair of RL with constraint types mentioned above and $\text{type}\in\{\mathit{\mathit{DP}},\mathit{\mathit{EqOpt}}\}$. For simplicity, we will omit the supscript ``type" when it is clear from the context and use $\bpi^*=(\pi^{*\alpha},\pi^{*\beta})$. 

For the fairness constraints, we consider the violation for each type of constraint in episode $k$ as the following,
$$\cC_{\mathrm{reg}}^{\mathit{DP}}(k)=\frac{1}{H}\sum_{h=1}^H \big|\bP^{\pi^{\alpha}_k,p^{*\alpha}}(a^\alpha_{k,h}=1)-\bP^{\pi^\beta_k,p^{*\beta}}(a^\beta_{k,h}=1)\big|,$$
and 
\begin{align*}
 \cC_{\mathrm{\mathrm{reg}}}^{\mathit{\mathit{EqOpt}}}(k)=\frac{1}{H}\sum_{h=1}^H \big|\bP^{\pi^{\alpha}_k,p^{*\alpha}}(a^\alpha_{k,h}=1\big|y^\alpha_{k,h}=1)-\bP^{\pi^\beta_k,p^{*\beta}}(a^\beta_{k,h}=1|y^\beta_{k,h}=1)\big|.  
\end{align*}
%$$\cC_{\mathrm{reg}}^{\mathit{EqOpt}}(k)=\frac{1}{H}\sum_{h=1}^H |\bP^{\pi^{\alpha}_k,p^{*\alpha}}(a^\alpha_{k,h}=1|y^\alpha_{k,h}=1)-\bP^{\pi^\beta_k,p^{*\beta}}(a^\beta_{k,h}=1|y^\beta_{k,h}=1)|.$$
The theoretical guarantees hold for any episode, not just the last episode.





\subsection{Choice of various of quantities} \label{subsec:theory}
In this part, we provide a formal theoretical guarantee for the performance of our algorithms under the previously mentioned criteria with suitably chosen quantities $\{\hat b^\vartheta_k\}_k$, $\{\hat c_k\}_k$, and $\{\hat d_k\}_k$, for each episode $k$. 

\paragraph{$Q$ and $V$ functions.} Two of the mostly used concepts in RL are $Q$ and $V$ functions. Specifically, $Q$ functions track the expected reward when a learner starts from state $s\in\cS$. Meanwhile, $V$ functions are the corresponding expected $Q$ functions of the selected action. For a reward function $r$ and a transition function $p$, the $Q$ and $V$ functions are defined as:
\begin{align*}
Q^{\pi,p}_r(s,a,h)&=r(s,a)+\sum_{s'\in\cS}p(s'|s,a)V^{\pi,p}_r(s',h+1),\\
V^{\pi,p}_r(s,h)&=\bE_{a\sim\pi(\cdot|s)}[Q^{\pi,p}_r(s,a,h)],
\end{align*}
where we set $V^{\pi,p}_r(s,H+1)=0$.

%=============
\paragraph{Choice of $\hat b^\vartheta_k$.} For $\{\hat b^\vartheta_k\}_k$, similar to \cite{brantley2020constrained}, we need $\{\hat b^\vartheta_k\}_k$ to be valid. 
\begin{definition}[Validity]
A bonus $\hat b^\vartheta_k$ is valid for episode $k$ if for all $(s,a)\in\cS\times\cA$ and $h\in[H]$,
\begin{align*}
&\Big |\hat r^\vartheta_k(s,a)-r^{*\vartheta}_k(s,a)+\sum_{s'\in\cS}\Big( p^\vartheta_k(s'|s,a)- p^{*\vartheta}(s'|s,a)\Big)
V^{\pi^{*\vartheta},p^{*\vartheta}}_{r^{*\vartheta}}(s',h+1)\Big|\le \hat b^\vartheta_k(s,a).
\end{align*}
\end{definition}

%\dcp{did you mean ``is valid for episode $k$"? Also,  I don't think $V$ is defined yet, and I thought there would be a $h$ as well as a $h+1$ somewhere in the math.}
Following the exporation-bonus setting~\cite{brantley2020constrained}, we set $\hat b^\vartheta_k=\min\Big\{2H,2H\sqrt{\frac{2\ln(16SAHk^2/\delta)}{N^\vartheta_k(s,a)}}\Big\}$, and have the following lemma.
\begin{lemma}\label{lm:b_k}
With probability at least $1-\delta$, for
$$\hat{b}^\vartheta_k(s,a)=\min\Big\{2H,2H\sqrt{\frac{2\ln(16SAHk^2/\delta)}{N^\vartheta_k(s,a)}}\Big\},$$ 
the bonus $\hat b^{\vartheta}_k(s,a)$ is valid for every  episode $k$ simultaneously.
\end{lemma}

\paragraph{Choice of $\hat c_{k,h}$ and $\hat d_{k,h}$.} For $\{\hat c_{k,h}\}_{k,h}$ and $\{\hat d_{k,h}\}_{k,h}$, we require them to be \textit{compatible}. 
\begin{definition}[Compatibility]
The sequence $\{\hat c_{k,h}\}_{k,h}$ is {\em compatible} if for all $h\in[H], k\in[K],$ $$|\bP^{\pi^{*\alpha},p_k^{\alpha}}(a_h=1)-\bP^{\pi^{*\beta},p_k^{\beta}}(a_h=1)|\le \hat c_{k,h}.$$
%\begin{equation*}
%|\bP^{\pi^{*\alpha},p_k^{\alpha}}(a_h=1)-\bP^{\pi^{*\beta},p_k^{\beta}}(a_h=1)|\le \hat c_{k,h}
%\end{equation*}
%
The sequence $\{\hat d_{k,h}\}_{k,h}$ is {\em compatible} if for all $h\in[H], k\in[K]$, $$|\bP^{\pi^{*\alpha},p_k^{\alpha}}(a_h=1|y_h=1)-\bP^{\pi^{*\beta},p_k^{\beta}}(a_h=1|y_h=1)|\le \hat d_{k,h}.$$
%\begin{equation*}
%|\bP^{\pi^{*\alpha},p_k^{\alpha}}(a_h=1|y_h=1)-\bP^{\pi^{*\beta},p_k^{\beta}}(a_h=1|y_h=1)|\le \hat d_{k,h}
%\end{equation*}
\end{definition}


Briefly speaking, we hope that when substituting $p^{*\vartheta}$ to $p^{\vartheta}_k$, that $\hat c_{k,h}$ and $\hat d_{k,h}$ can control the fairness constraints violation. %We first consider $\hat c_{k,h}$, notice $\bP^{\pi^{*\alpha},p^{*\alpha}}(a_h=1)=\bP^{\pi^{*\beta},p^{*\beta}}(a_h=1)$, then by triangular inequality, 
%\begin{align*}
% &|\bP^{\pi^{*\alpha},p_k^{\alpha}}(a_h=1)-\bP^{\pi^{*\beta},p_k^{\beta}}(a_h=1)|\\
% &\le \sum_{\vartheta\in\{\alpha,\beta\}} |\bP^{\pi^{*\vartheta},p_k^{\vartheta}}(a_h=1)-\bP^{\pi^{*\vartheta},p^{*\vartheta}}(a_h=1)|.
%\end{align*}
%Thus, it is sufficient to choose $\hat c_{k,h}$ to bound $\sum_{\vartheta} |\bP^{\pi^{*\vartheta},p_k^{\vartheta}}(a_h=1)-\bP^{\pi^{*\vartheta},p^{*\vartheta}}(a_h=1)|$.
Let us use $S$ to denote $|\cS|$ and $A$ to denote $|\cA|$.
%
\begin{lemma}\label{lm:c_kd_k}
Denote $N^{\vartheta,\min}_{k}=\min_{s,a}N^\vartheta_k(s,a)$. For any $\{\epsilon_k\}_{k=1}^K$, with probability at least $1-\delta$, we take
$$\hat c_{k,h}=\sum_{\vartheta\in\{\alpha,\beta\}}H\sqrt{\frac{2S\ln(16SAHk^2/(\epsilon_k\delta))}{N^{\vartheta,\min}_{k}}}+2\epsilon_k HS.$$
Then, the sequence $\{\hat c_{k,h}\}_{k,h}$ is compatible.
\end{lemma}
Similarly, for $\hat d_{k,h}$, we have the following lemma. 
%\begin{lemma}\label{lm:d2}
%Under Assumption~\ref{ass:p2}, for any $\epsilon>0$, if $\hat p$ with probability at least $1-\delta$, 
%$$\hat d_{k,h}=,$$
%$\hat d_{k,h}$ is compatible for all $h\in[H]$ and $k\in[K]$.
%\end{lemma}
\begin{lemma}\label{lm:d}
Denote $p^{\vartheta,\min}_{k}=\min_{s,a}p^\vartheta_k(y=1|s,a)$. For any $\{\epsilon_k\}_{k=1}^K$, with probability at least $1-\delta$, we take
%$$\hat d_{k,h}=\sum_{\vartheta}\frac{4H\sqrt{\frac{2S\ln(8SAk^2/(\epsilon\delta))}{N^{\vartheta,\min}_{k}}}+4\epsilon HS}{p^{\vartheta,\min}_{k}\left(p^{\vartheta,\min}_{k}-\sqrt{\frac{4\ln 2+2\ln(SAk^2/\delta)}{N^{\vartheta,\min}_{k}}}\right)}.,$$
$$\hat d_{k,h}=\sum_{\vartheta\in\{\alpha,\beta\}}\frac{3H\sqrt{\frac{2S\ln(32SAk^2/(\epsilon_k\delta))}{N^{\vartheta,\min}_{k}}}+3\epsilon_k HS}{p^{\vartheta,\min}_{k}\left(p^{\vartheta,\min}_{k}-\sqrt{\frac{4\ln 2+2\ln(4SAk^2/\delta)}{N^{\vartheta,\min}_{k}}}\right)}$$
if $p^{\vartheta,\min}_{k}>\sqrt{\frac{4\ln 2+2\ln(4SAk^2/\delta)}{N^{\vartheta,\min}_{k}}}$; Otherwise, we set $\hat d_{k,h}=1$.
%$$\hat d_{k,h}=\left\{\begin{matrix}
	%\sum_{\vartheta}\frac{3H\sqrt{\frac{2S\ln(%16SAk^2/(\epsilon_k\delta))}{N^{\vartheta,min}_{k}}}+3\epsilon_k HS}{p^{\vartheta,min}_{k}\left(p^{\vartheta,min}_{k}-\sqrt{\frac{4\ln 2+2\ln(2SAk^2/\delta)}{N^{\vartheta,min}_{k}}}\right)} ,&\text{if}~p^{\vartheta,min}_{k}>\sqrt{\frac{4\ln 2+2\ln(2SAk^2/\delta)}{N^{\vartheta,min}_{k}}};\\ 
%	1,&\text{otherwise};
%\end{matrix}\right.$$
Then, the sequence $\{\hat d_{k,h}\}_{k,h}$ is compatible.
\end{lemma}


%Notice that Assumption~\ref{ass:p} is usually for theoretical purpose only in the RL literature, and $c$ is a quantity that is commonly not observable, which cannot help us design practical algorithms given that we cannot ensure.... However, the following assumption can imply Assumption~\ref{ass:p}, and can be estimated and help design practical algorithm.





%=============
\subsection{Main theorems}

In this subsection, we provide our formal theoretical guarantees for the reward regret and fairness constraints violation. We require technical Assumption~\ref{ass:kernel}.
%
%Recall that we are optimizing policy over $\Pi_k$ for the $k$-th episode, which can guarantee that we have $\bP^{\pi_k,p^\vartheta_k}(s_{k,h}=s,a_{k,h}=a)\ge \eta^{type}_k$ for all $s,a,h$ and $type\in\{DP, EqOpt\}$. 
%
\begin{assumption}\label{ass:kernel}
(a). For all $(s,a,s')\in\cS\times\cA\times\cS$, there exists a universal constant $C>0$, such that $p^{*\vartheta}(s'|s,a)\ge C$ for $\vartheta=\{\alpha,\beta\}$. (b). For all $(x,a)\in\cX\times\cA$, there exists a universal constant $\tilde C$, such that $\pi^{*\vartheta}(a|x)\ge \tilde C$.
\end{assumption}
Assumption~\ref{ass:kernel}  implies irreducibility of the Markov process and  ensures feasibility of our
optimization problems (see Appendix~\ref{app:feasibility}). 
%
Recall that at episode $k\in[K]$, for each group $\vartheta$, we have $n^\vartheta_{k}\ge 1$ individuals drawn for each group $\vartheta$. %Let us denote $\min_{t\in[k]\vartheta\in\{\alpha,\beta\}}n^\vartheta_t=n_k$. 
And as a concrete exemplified choice of $\eta_k$ and $\epsilon_k$, we take $\eta_k=k^{-\frac{1}{3}}$ and $\epsilon_k=(kHS)^{-1}$. 

\paragraph{Reward regret.} For the reward regret, for either demographic parity or equalized opportunity, we can provide the following theoretical guarantee. Recall for two positive sequences $\{a_j\}$ and $\{b_j\}$, we write $a_j =\cO(b_j)$ if $\lim_{j\rightarrow\infty}(a_j/b_j) < \infty$. 

\begin{theorem}\label{thm:reward}
For $type\in\{\mathit{DP},\mathit{EqOpt}\}$, with probability at least $1-\delta$, there exists a threshold $T=\cO\left(\Big(\frac{H\ln(SA/\delta)}{n_k}\Big)^{3}\right)$, such that for all $k\ge T$,
$$\cR^{\text{type}}_{\mathrm{reg}}(k)=\cO\left(Hk^{-\frac{1}{3}}\sqrt{HS\ln(S^2AH^2k^3/\delta)}\right).$$
\end{theorem}

By Theorem~\ref{thm:reward}, our algorithms for each of the group fairness notions can ensure vanishing reward regrets when $k$ goes to infinity, which implies that the performance in regard to regret reward improves as the number of episodes increases.

\paragraph{Fairness constraints violation.} For fairness violation, we have the following Theorem~\ref{thm:constraint}.
%
\begin{theorem}\label{thm:constraint}
For $type\in\{\mathit{DP},\mathit{EqOpt}\}$, with probability at least $1-\delta$, there exists a threshold $T=\cO\left(\Big(\frac{H\ln(SA/\delta)}{n_k}\Big)^{3}\right)$, such that for all $k\ge T$,
$$\cC_{\mathrm{reg}}^{\text{type}}(k)\le \cO\left( k^{-\frac{1}{3}}\sqrt{SH\ln(S^2HAk^3/\delta)}\right).$$
\end{theorem}

By Theorem~\ref{thm:constraint},  our algorithms for each of the group fairness notions can ensure vanishing fairness violation when $k$ goes to infinity, which implies the performance in regard to fairness violations improves as  the number of episodes increases.














\iffalse
But for equalized opportunity, it is a bit more complicated to build theory due to the existence of conditional probability, i.e. we need to bound the denominator in calculating conditional probability under $\bP^{\pi^{*\vartheta},p^{*\vartheta}}$  away from $0$. In RL literature, this type of reachability is commonly assumed in the RL literature \cite{xx}. \zhun{say more about that, consult with other people}

\begin{assumption} \label{ass:p2}
For all $h\in H,k\in[K]$, and $\vartheta\in\{\alpha,\beta\}$, there exists a universal constant $c>0$, such that
$$\bP^{\pi^{*\vartheta},p^{*\vartheta}}(y^\vartheta_{k,h}=1)\ge c.$$
\end{assumption}
Notice that Assumption~\ref{ass:p2} is usually for theoretical purpose only in the RL literature, and $c$ is a quantity that is commonly not observable/estimable, which cannot help us to design practical algorihtms. On the other hand, the following assumption can imply Assumption~\ref{ass:p2}, and can be estimated and help design practical quantities used in algorithms as in Lemma~\ref{lm:d}. Given that, we have the following lemma.


\begin{assumption} \label{ass:p}
For all $(s,a)\in\cS\times\cA$, $p^{*\vartheta}(y=1|s,a)$ is bounded away from $0$. In other words, there exists a universal constant $\tilde{c}>0$, such that
$$p^{*\vartheta}(y=1|s,a)\ge \tilde c.$$
Moreover, the above formula further implies 
$$\bP^{\pi^{*\vartheta},p^{*\vartheta}}(y_{k,h}=1)\ge \tilde c.$$
\end{assumption}
The above assumption \zhun{add interpretation} \zhun{scale right?} We \textbf{do not} need to know the exact value of $\tilde c$. Most importantly, we can derive the following lemma.
\fi
























==> conclusion.tex <==
\section{Conclusions}
